gSeaGen code by KM3NeT: an efficient tool to propagate muons simulated with CORSIKA

The KM3NeT Collaboration has tackled a common challenge faced by the astroparticle physics community, namely adapting the experiment-specific simulation software to work with the CORSIKA air shower simulation output. The proposed solution is an extension of the open source code gSeaGen, which allows the transport of muons generated by CORSIKA to a detector of any size at an arbitrary depth. The gSeaGen code was not only extended in terms of functionality but also underwent a thorough redesign of the muon propagation routine, resulting in a more accurate and efficient simulation. This paper presents the capabilities of the new gSeaGen code as well as prospects for further developments.

==> authorlist_for_arxiv.tex <==
S.~Aiello, A.~Albert, A.\,R.~Alhebsi, M.~Alshamsi, S. Alves Garre, A. Ambrosone, F.~Ameli, M.~Andre, L.~Aphecetche, M. Ardid, S. Ardid, H.~Atmani, J.~Aublin, F.~Badaracco, L.~Bailly-Salins, Z. Barda\v{c}ov\'{a}, B.~Baret, A. Bariego-Quintana, Y.~Becherini, M.~Bendahman, F.~Benfenati, M.~Benhassi, M.~Bennani, D.\,M.~Benoit, E.~Berbee, V.~Bertin, S.~Biagi, M.~Boettcher, D.~Bonanno, A.\,B.~Bouasla, J.~Boumaaza, M.~Bouta, M.~Bouwhuis, C.~Bozza, R.\,M.~Bozza, H.Br\^{a}nza\c{s}, F.~Bretaudeau, M.~Breuhaus, R.~Bruijn, J.~Brunner, R.~Bruno, E.~Buis, R.~Buompane, J.~Busto, B.~Caiffi, D.~Calvo, A.~Capone, F.~Carenini, V.~Carretero, T.~Cartraud, P.~Castaldi, V.~Cecchini, S.~Celli, L.~Cerisy, M.~Chabab, A.~Chen, S.~Cherubini, T.~Chiarusi, M.~Circella, R.~Cocimano, J.\,A.\,B.~Coelho, A.~Coleiro, A. Condorelli, R.~Coniglione, P.~Coyle, A.~Creusot, G.~Cuttone, R.~Dallier, A.~De~Benedittis, B.~De~Martino, G.~De~Wasseige, V.~Decoene, I.~Del~Rosso, L.\,S.~Di~Mauro, I.~Di~Palma, A.\,F.~D\'\i{}az, D.~Diego-Tortosa, C.~Distefano, A.~Domi, C.~Donzaud, D.~Dornic, E.~Drakopoulou, D.~Drouhin, J.-G. Ducoin, R. Dvornick\'{y}, T.~Eberl, E. Eckerov\'{a}, A.~Eddymaoui, T.~van~Eeden, M.~Eff, D.~van~Eijk, I.~El~Bojaddaini, S.~El~Hedri, V.~Ellajosyula, A.~Enzenh\"ofer, G.~Ferrara, M.~D.~Filipovi\'c, F.~Filippini, D.~Franciotti, L.\,A.~Fusco, S.~Gagliardini, T.~Gal, J.~Garc{\'\i}a~M{\'e}ndez, A.~Garcia~Soto, C.~Gatius~Oliver, N.~Gei{\ss}elbrecht, E.~Genton, H.~Ghaddari, L.~Gialanella, B.\,K.~Gibson, E.~Giorgio, I.~Goos, P.~Goswami, S.\,R.~Gozzini, R.~Gracia, C.~Guidi, B.~Guillon, M.~Guti{\'e}rrez, C.~Haack, H.~van~Haren, A.~Heijboer, L.~Hennig, J.\,J.~Hern{\'a}ndez-Rey, W.~Idrissi~Ibnsalih, G.~Illuminati, D.~Joly, M.~de~Jong, P.~de~Jong, B.\,J.~Jung, P.~Kalaczy\'nski, G.~Kistauri, C.~Kopper, A.~Kouchner, Y. Y. Kovalev, V.~Kueviakoe, V.~Kulikovskiy, R.~Kvatadze, M.~Labalme, R.~Lahmann, M.~Lamoureux, G.~Larosa, C.~Lastoria, A.~Lazo, S.~Le~Stum, G.~Lehaut, V.~Lema{\^\i}tre, E.~Leonora, N.~Lessing, M.~Lindsey~Clark, F.~Longhitano, F.~Magnani, J.~Majumdar, L.~Malerba, F.~Mamedov, J.~Ma\'nczak, A.~Manfreda, M.~Marconi, A.~Margiotta, A.~Marinelli, C.~Markou, L.~Martin, M.~Mastrodicasa, S.~Mastroianni, J.~Mauro, G.~Miele, P.~Migliozzi, E.~Migneco, M.\,L.~Mitsou, C.\,M.~Mollo, L. Morales-Gallegos, A.~Moussa, I.~Mozun~Mateo, R.~Muller, M.\,R.~Musone, M.~Musumeci, S.~Navas, A.~Nayerhoda, C.\,A.~Nicolau, B.~Nkosi, B.~{\'O}~Fearraigh, V.~Oliviero, A.~Orlando, E.~Oukacha, D.~Paesani, J.~Palacios~Gonz{\'a}lez, G.~Papalashvili, V.~Parisi, E.J. Pastor Gomez, C.~Pastore, A.~M.~P{\u a}un, G.\,E.~P\u{a}v\u{a}la\c{s}, S. Pe\~{n}a Mart\'inez, M.~Perrin-Terrin, V.~Pestel, R.~Pestes, P.~Piattelli, A.~Plavin, C.~Poir{\`e}, V.~Popa, T.~Pradier, J.~Prado, S.~Pulvirenti, C.A.~Quiroz-Rangel, N.~Randazzo, S.~Razzaque, I.\,C.~Rea, D.~Real, G.~Riccobene, J.~Robinson, A.~Romanov, E.~Ros, A. \v{S}aina, F.~Salesa~Greus, D.\,F.\,E.~Samtleben, A.~S{\'a}nchez~Losa, S.~Sanfilippo, M.~Sanguineti, D.~Santonocito, P.~Sapienza, J.~Schnabel, J.~Schumann, H.~M. Schutte, J.~Seneca, I.~Sgura, R.~Shanidze, A.~Sharma, Y.~Shitov, F. \v{S}imkovic, A.~Simonelli, A.~Sinopoulou, B.~Spisso, M.~Spurio, D.~Stavropoulos, I. \v{S}tekl, S.\,M.~Stellacci, M.~Taiuti, Y.~Tayalati, H.~Thiersen, S.~Thoudam, I.~Tosta~e~Melo, B.~Trocm{\'e}, V.~Tsourapis, A. Tudorache, E.~Tzamariudaki, A.~Ukleja, A.~Vacheret, V.~Valsecchi, V.~Van~Elewyck, G.~Vannoye, G.~Vasileiadis, F.~Vazquez~de~Sola, A. Veutro, S.~Viola, D.~Vivolo, A. van Vliet, E.~de~Wolf, I.~Lhenry-Yvon, S.~Zavatarelli, A.~Zegarelli, D.~Zito, J.\,D.~Zornoza, J.~Z{\'u}{\~n}iga, N.~Zywucka
